Planar Reachability Under Single Vertex or Edge Failures

In this paper we present an efficient reachability oracle under single-edge or single-vertex failures for planar directed graphs. Specifically, we show that a planar digraph $G$ can be preprocessed in $O(n\log^2{n}/\log\log{n})$ time, producing an $O(n\log{n})$-space data structure that can answer in $O(\log{n})$ time whether $u$ can reach $v$ in $G$ if the vertex $x$ (the edge~$f$) is removed from $G$, for any query vertices $u,v$ and failed vertex $x$ (failed edge $f$). To the best of our knowledge, this is the first data structure for planar directed graphs with nearly optimal preprocessing time that answers all-pairs queries under any kind of failures in polylogarithmic time. We also consider 2-reachability problems, where we are given a planar digraph $G$ and we wish to determine if there are two vertex-disjoint (edge-disjoint) paths from $u$ to $v$, for query vertices $u,v$. In this setting we provide a nearly optimal 2-reachability oracle, which is the existential variant of the reachability oracle under single failures, with the following bounds. We can construct in $O(n\log^{O(1)}{n})$ time an $O(n\log^{3+o(1)}{n})$-space data structure that can check in $O(\log^{2+o(1)}{n})$ time for any query vertices $u,v$ whether $v$ is 2-reachable from $u$, or otherwise find some separating vertex (edge) $x$ lying on all paths from $u$ to $v$ in $G$. To obtain our results, we follow the general recursive approach of Thorup for reachability in planar graphs [J.~ACM~'04] and we present new data structures which generalize dominator trees and previous data structures for strong-connectivity under failures [Georgiadis et al., SODA~'17]. Our new data structures work also for general digraphs and may be of independent interest.

==> omitted.tex <==
\section{Omitted Proofs}\label{s:omitted}
\suppressedset*
\begin{proof}
  We apply induction on the level of the recursive call
  that is passed graph $G$ with suppressed set $\supr$.
  In the first recursive call (level $0$) after applying Lemma~\ref{l:layered},
  $\supr$ has size at most $1$.
  
  Let the level of the recursive call be at least $1$.
  In the parent call the suppressed set $\supr'$ had size at most $5$.
  If $|\supr'|=5$, then the balanced cycle separator $C_{ab}$ put at most $3$
  vertices of $\supr'$ strictly on one side of $C_{ab}$.
  Since the entire set $V(C_{ab})$ was subsequently contracted
  into a single vertex that got suppressed, $\supr$ has size at most $3+1=4$.
  
  On the other hand, if $|\supr'|\leq 4$, then clearly $|\supr|\leq |\supr'|+1\leq 5$.
\end{proof}

\recursionlevels*
\begin{proof}
  If the cycle separator computed at the parent call balanced all the vertices
  of the graph $G'$ with suppressed set $A'$ and $n$ vertices, then $G$ has at most $\frac{3}{4}n+1$
  vertices.

  However, if $|A'|=5$, then $G$ might have nearly $n$ vertices.
  But in this case $|A|\leq 4$, so the in the children recursive
  calls the graphs will certainly have no more than $\frac{3}{4}n$ vertices.

  This proves that at each recursive call the number of vertices is
  reduced by a constant factor compared to the grandparent call,
  i.e., the depth of the recursion tree is $O(\log{n})$.
\end{proof}

\singleface*
\begin{proof}
Since $C_{ab}$ is a cycle separator, 
we can also view $C_{ab}$ as a closed curve
that does not cross any edges (but can follow the edges)
  of $G-A$ and has (the embedding of) each $P_i$ as a contiguous part.
  After removing vertices $V(S_{ab})\setminus V(P_i)$
  from $G-A$, the part of the curve that does
  not correspond to $P_i$ connects the endpoints
  of $P_i$ and does not intersect
  (the embedding of) any other vertices or edges of $G[\bar{V_i}]-A$.
  Hence, this part lies inside
  a single face of the component of $G[\bar{V_i}]-A$
  that contains $P_i$.
  We conclude that the endpoints of $P_i$
  lie on that single face.
\end{proof}


